OSTAF: A One-Shot Tuning Method for Improved Attribute-Focused T2I Personalization

Personalized text-to-image (T2I) models not only produce lifelike and varied visuals but also allow users to tailor the images to fit their personal taste. These personalization techniques can grasp the essence of a concept through a collection of images, or adjust a pre-trained text-to-image model with a specific image input for subject-driven or attribute-aware guidance. Yet, accurately capturing the distinct visual attributes of an individual image poses a challenge for these methods. To address this issue, we introduce OSTAF, a novel parameter-efficient one-shot fine-tuning method which only utilizes one reference image for T2I personalization. A novel hypernetwork-powered attribute-focused fine-tuning mechanism is employed to achieve the precise learning of various attribute features (e.g., appearance, shape or drawing style) from the reference image. Comparing to existing image customization methods, our method shows significant superiority in attribute identification and application, as well as achieves a good balance between efficiency and output quality.

==> Tex/figs_tex/fig_simple_exp.tex <==
\begin{figure}
    \includegraphics[width=0.5\textwidth]{Tex/assets/simple_exp.pdf}
    \caption{For the same reference image, we fine-tune both the encoder and decoder separately, obtaining two distinct sets of results.}
    \label{fig:simple_exp}
\end{figure}



==> Tex/figs_tex/material/code.tex <==

\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{Tex/assets/Material/code.pdf}
    \caption{ Detailed training parameter configurations for attribute-focused customization.}
    \label{fig:code}
\end{figure*}


==> Tex/figs_tex/visual_encoder.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{articles/assets/visual_encoder.pdf}
    \caption{The architecture of visual encoder.}
    \label{fig:encoder}
\end{figure}




==> Tex/table/table_style.tex <==

\begin{table*}[]
\centering
\caption{Quantitative comparison with respect to Prospect for style attribute customization.}
\label{tab:style_compare}
\begin{tabular}{c|cc}
\hline
Metric   & \multicolumn{2}{c}{Style Customization}            \\ \hline
Method   & Gram Matrics  $\downarrow$ & User Study $\uparrow$ \\ \hline
Prospect\cite{zhang2023prospect} & 0.0611                     &              \\ \hline
Ours     &\textbf{0.0340}                  &                       \\ \hline
\end{tabular}
\end{table*}



